Averaging Orientations with Molecular Symmetry in Cryo-EM

Cryogenic electron microscopy (cryo-EM) is an invaluable technique for determining high-resolution three-dimensional structures of biological macromolecules using transmission particle images. The inherent symmetry in these macromolecules is advantageous, as it allows each image to represent multiple perspectives. However, data processing that incorporates symmetry can inadvertently average out asymmetric features. Therefore, a key preliminary step is to visualize 2D asymmetric features in the particle images, which requires estimating orientation statistics under molecular symmetry constraints. Motivated by this challenge, we introduce a novel method for estimating the mean and variance of orientations with molecular symmetry. Utilizing tools from non-unique games, we show that our proposed non-convex formulation can be simplified as a semi-definite programming problem. Moreover, we propose a novel rounding procedure to determine the representative values. Experimental results demonstrate that the proposed approach can find the global minima and the appropriate representatives with a high degree of probability. We release the code of our method as an open-source Python package named pySymStat. Finally, we apply pySymStat to visualize an asymmetric feature in an icosahedral virus, a feat that proved unachievable using the conventional 2D classification method in RELION.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{subfig}
\usepackage{epstopdf}
% \usepackage{algorithmic}

\usepackage{amsmath}
% \usepackage{amsfonts}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
% \usepackage{graphicx}
\usepackage{booktabs}
\usepackage{siunitx}
\usepackage{verbatim}
\usepackage{enumerate}
% \usepackage{authblk}
\usepackage{afterpage}
\usepackage[misc]{ifsym}
\usepackage{setspace}
% \usepackage{geometry}
\usepackage{lineno}
%\usepackage{bibunits}
\usepackage{float}
\usepackage{color}
\usepackage{mathrsfs}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{threeparttable}
\usepackage{url}


% Add a serial/Oxford comma by default.
\newcommand{\Sort}[4]{\textbf{sort} #1 \textbf{into} #2 \textbf{by the value} #3 \textbf{in #4 order}}
\newcommand{\SortKMax}[4]{\textbf{sort} #1 \textbf{by the value} #4 and \textbf{transfer} the #2 maximum values \textbf{into} #3}
\newcommand{\Define}[2]{\textbf{define} #1 \textbf{as} #2}
\newcommand{\Assign}[2]{\textbf{assign} #1 \textbf{with} #2}
\newcommand{\Fill}[2]{\textbf{fill} #1 \textbf{into} #2}

\newcommand{\be}{\mathbf{e}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\rH}{\mathrm{H}}
\newtheorem{remark}[theorem]{Remark}

\newcommand{\code}{\textsf}

\usepackage[labelfont=bf, figurename = Figure, format = plain]{caption}

%\geometry{left=2.54cm, right=2.54cm, top=2.54cm, bottom=2.54cm}

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}

\graphicspath{{figures/}}

% Used for creating new theorem and remark environments
% \newsiamremark{remark}{Remark}
% \newsiamremark{hypothesis}{Hypothesis}
% \crefname{hypothesis}{Hypothesis}{Hypotheses}
% \newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Orientation Estimations Under Molecular Symmetry}{Q. Zhang, C. Bao, H. Lin, and M. Hu.}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{The Moments of Orientation Estimations Considering Molecular Symmetry in Cryo-EM\thanks{Submitted to the editors DATE.
\funding{CL Bao is supported by the National Key R\&D Program of China (No.2021YFA1001300), National Natural Science Foundation of China (No.12271291), Tsinghua University Initiative Scientific Research Program. MX Hu is supported by Advanced Innovation Center for Structural Biology and Beijing Frontier Research Center for Biological Structure.}}}

% Authors: full names plus addresses.
% \author{Dianne Doe\thanks{Imagination Corp., Chicago, IL
%   (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
% \and Paul T. Frank\thanks{Department of Applied Mathematics, Fictional University, Boise, ID
%   (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
% \and Jane E. Smith\footnotemark[3]}

\author{Qi Zhang\thanks{Key Laboratory of Protein Sciences (Tsinghua University), Ministry of Education, Beijing, China; School of Life Science, Tsinghua University, Beijing, China; Beijing Advanced Innovation Center for Structural Biology; Beijing Frontier Research Center for Biological Structure.}
\and Chenglong Bao\footnotemark[2]\textsuperscript{ ,}\thanks{Yau Mathematical Sciences Center, Tsinghua University, Beijing, China; Yanqi Lake Beijing Institute of Mathematical Sciences and Applications. (\email{clbao@mail.tsinghua.edu.cn})}
\and Hai Lin\thanks{Shing-Tung Yau Center of Southeast University, Southeast University, Nanjing, China; School of Mathematics, Southeast University, Nanjing, China (\email{hailinhl@gmail.com})}
\and Mingxu Hu\thanks{School of Life Science, Tsinghua University, Beijing, China; Beijing Advanced Innovation Center for Structural Biology; Beijing Frontier Research Center for Biological Structure. (\email{humingxu@mail.tsinghua.edu.cn})}}


% \author[1,2,3,4]{Qi Zhang}
% \author[5]{Chenglong Bao\textsuperscript{\textdagger}}
% \author[5,6]{Hai Lin\textsuperscript{\textdagger}}
% \author[1,2,3,4]{Mingxu Hu\textsuperscript{\textdagger}}
% \renewcommand{\thefootnote}{\fnsymbol{footnote}}
% \footnotetext[1]{Key Laboratory of Protein Sciences (Tsinghua University), Ministry of Education, Beijing, China}
% \footnotetext[2]{School of Life Science, Tsinghua University, Beijing, China}
% \footnotetext[3]{Beijing Advanced Innovation Center for Structural Biology}
% \footnotetext[4]{Beijing Frontier Research Center for Biological Structure}
% \footnotetext[5]{Yau Mathematical Sciences Center, Tsinghua University, Beijing, China}
% \footnotetext[6]{Department of Mathematical Sciences, Tsinghua University, Beijing, China}
% \affil[1]{Key Laboratory of Protein Sciences (Tsinghua University), Ministry of Education, Beijing, China}
% \affil[2]{School of Life Science, Tsinghua University, Beijing, China}
% \affil[3]{Beijing Advanced Innovation Center for Structural Biology}
% \affil[4]{Beijing Frontier Research Center for Biological Structure}
% \affil[5]{Yau Mathematical Sciences Center, Tsinghua University, Beijing, China}
% \affil[6]{Department of Mathematical Sciences, Tsinghua University, Beijing, China}

% \usepackage{amsopn}
% \DeclareMathOperator{\diag}{diag}


%% Added on Overleaf: enabling xr
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
  \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
  \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}
%%% END HELPER CODE
%%% Local Variables:
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End:

